Mask2Anomaly: Mask Transformer for Universal Open-set Segmentation

Segmenting unknown or anomalous object instances is a critical task in autonomous driving applications, and it is approached traditionally as a per-pixel classification problem. However, reasoning individually about each pixel without considering their contextual semantics results in high uncertainty around the objects' boundaries and numerous false positives. We propose a paradigm change by shifting from a per-pixel classification to a mask classification. Our mask-based method, Mask2Anomaly, demonstrates the feasibility of integrating a mask-classification architecture to jointly address anomaly segmentation, open-set semantic segmentation, and open-set panoptic segmentation. Mask2Anomaly includes several technical novelties that are designed to improve the detection of anomalies/unknown objects: i) a global masked attention module to focus individually on the foreground and background regions; ii) a mask contrastive learning that maximizes the margin between an anomaly and known classes; iii) a mask refinement solution to reduce false positives; and iv) a novel approach to mine unknown instances based on the mask-architecture properties. By comprehensive qualitative and qualitative evaluation, we show Mask2Anomaly achieves new state-of-the-art results across the benchmarks of anomaly segmentation, open-set semantic segmentation, and open-set panoptic segmentation.

==> tab-backboneSize.tex <==
\begin{table*}[!ht]
\centering
\renewcommand{\arraystretch}{1.15}
\resizebox{1\linewidth}{!}{\begin{tabular}{c|cc|cc|cc|cc|cc|cc}
\multicolumn{1}{c|}{}&\multicolumn{2}{c|}{SMIYC RA-21}&\multicolumn{2}{c|}{SMIYC RO-21}&\multicolumn{2}{c|}{FS L\&F}&\multicolumn{2}{c|}{FS Static}&\multicolumn{2}{c|}{Road Anomaly}& \multicolumn{2}{c}{Average}\\
\cline{2-3}\cline{4-5}\cline{6-7}\cline{8-9}\cline{10-11}\cline{12-13}
\multicolumn{1}{c|}{Backbone}&\multicolumn{1}{c|}{AuPRC $\uparrow$}&\multicolumn{1}{c|}{FPR$_{95}$ $\downarrow$}&\multicolumn{1}{c|}{AuPRC $\uparrow$} &\multicolumn{1}{c|}{FPR$_{95}$ $\downarrow$}&\multicolumn{1}{c|}{AuPRC $\uparrow$} &\multicolumn{1}{c|}{FPR$_{95}$ $\downarrow$}&\multicolumn{1}{c|}{AuPRC $\uparrow$} &\multicolumn{1}{c|}{FPR$_{95}$ $\downarrow$}&\multicolumn{1}{c|}{AuPRC $\uparrow$} &\multicolumn{1}{c|}{FPR$_{95}$ $\downarrow$}&\multicolumn{1}{c|}{AuPRC $\uparrow$} &\multicolumn{1}{c}{FPR$_{95}$$\downarrow$}\\
\Xhline{3\arrayrulewidth}

Swin-Tiny &53.61 &31.2 &78.58 &2.56 &44.81 &43.46 &77.99 &9.96 &63.75 &28.75 &63.74 &23.18\\		

Swin-Small &70.84 &34.16 &92.66 &0.47 &55.59 &15.11 &87.76 &4.96 &75.88 &19.19 &76.54 &14.77\\	

Swin-Base &94.9 &4.38 &95.21 &0.28 &65.57 &5.37 &88.51 &5.2 &84.46 &9.26 &\textbf{85.73} &\textbf{4.89} \\

Swin-Large &77.4 &25.06 &96.95 &0.151 &66.82 &4.61 &91.26 &6.02 &75.48 &9.88 &81.50 &9.14 \\

\end{tabular}}
\caption{\textbf{Performance on Larger Backbone:} Shows the performance of~\our{} on various backbone size.~\our{} with Swin-base backbone gives the best performance.} \vspace{-1em}
\label{tab:backbone-size} 
\end{table*}
